Temporal Regularization Makes Your Video Generator Stronger

Temporal quality is a critical aspect of video generation, as it ensures consistent motion and realistic dynamics across frames. However, achieving high temporal coherence and diversity remains challenging. In this work, we explore temporal augmentation in video generation for the first time, and introduce FluxFlow for initial investigation, a strategy designed to enhance temporal quality. Operating at the data level, FluxFlow applies controlled temporal perturbations without requiring architectural modifications. Extensive experiments on UCF-101 and VBench benchmarks demonstrate that FluxFlow significantly improves temporal coherence and diversity across various video generation models, including U-Net, DiT, and AR-based architectures, while preserving spatial fidelity. These findings highlight the potential of temporal augmentation as a simple yet effective approach to advancing video generation quality.

==> sec/1_intro_bak.tex <==
\section{Introduction}
\label{sec:intro}


The pursuit of photorealistic video generation faces a critical dilemma: while spatial synthesis (\textit{e.g.}, Stable Diffusion-series \cite{rombach2022high, esser2024scaling}) has achieved remarkable fidelity, temporal coherence remains an elusive target. Modern video generators, whether diffusion-based \cite{kong2024hunyuanvideo, zheng2024open, li2025minimax, yang2024cogvideox} or autoregressive \cite{deng2024autoregressive, hong2022cogvideo, wang2024emu3}, often produce sequences with inconsistent motion (\textit{e.g.}, flickering textures, discontinuous object trajectories) or repetitive dynamics (\textit{e.g.}, cyclic limb movements).
% Traditional spatial augmentations like CutMix \cite{yun2019cutmix} or Mixup \cite{zhang2017mixup}, though effective for images, fail to address this temporal brittleness—a critical shortcoming, as videos inherently require models to reason about dynamics rather than static patterns. This gap in sequential-data regularization manifests concretely as temporal overfitting, where generators rigidly replicate observed motion trajectories instead of learning generalizable physics.
These artifacts stem from a fundamental limitation: \textcolor{red}{models overfit to rigid temporal patterns in training data, memorizing specific motion sequences (\textit{e.g.}, ``walking left-to-right") rather than learning generalized dynamics.} While spatial augmentations \cite{yun2019cutmix, zhang2017mixup} mitigate overfitting in static images/frames, they fail to address temporal brittleness—a critical shortcoming, as videos inherently require reasoning about state transitions rather than isolated frames.


To formalize this issue, we observe that video generation demands modeling two interrelated factors: (a) Spatial realism: Textures, lighting, and object shapes in individual frames. (b) Temporal plausibility: Physically coherent transitions between frames.
Modern architectures excel at spatial realism by leveraging large-scale image priors \cite{rombach2022high, esser2024scaling, sun2024autoregressive}, yet struggle with temporal plausibility due to limited video datasets. For instance, models trained on short clips (\textit{e.g.}, 16 frames) often ``memorize" motion trajectories (\textit{e.g.}, fixed walking speed/direction) rather than learning generalized dynamics \cite{chen2023videocrafter1, chen2024videocrafter2}. This manifests as:
\ding{182} \textbf{\textit{Temporal overfitting}}: Rigid replication of observed motion paths.
\ding{183} \textbf{\textit{Distributional fragility}}: Failure to generalize to novel trajectories.
Current solutions, such as motion-content decomposition \cite{}, rely on architectural modifications but neglect the root cause: insufficient temporal diversity during training. Spatial augmentations like cropping or color jittering \cite{} perturb pixels but leave temporal correlations intact, allowing models to exploit spurious shortcuts (\textit{e.g.}, ``frame \#5 must follow \#4").



In this paper, we propose \textbf{FluxFlow}, a data augmentation strategy that injects controlled temporal perturbations into video generation training. Inspired by human cognition—where we infer missing frames or reorder events—FluxFlow operates on a simple principle: \textbf{\textit{disrupting fixed temporal order to force the model to learn disentangled motion/optical flow dynamics}}. At its core, FluxFlow applies \textit{frame shuffling} with adaptive constraints:
% \begin{itemize}[leftmargin=*]
%     \item[$\blacktriangleright$] \textbf{Local shuffling}: Swap frames within a random selection (\textit{e.g.}, random shuffle 2 inconsecutive frames).
%     \item[$\blacktriangleright$] \textbf{Curriculum scheduling}: Gradually increase shuffle intensity as training progresses.
% \end{itemize}
(\textit{i}) Local shuffling: Swap frames within a random selection (\textit{e.g.}, random shuffle two inconsecutive frames). (\textit{ii}) Curriculum scheduling: Gradually increase shuffle intensity as training progresses.
\textcolor{red}{This strategy acts as a \textbf{temporal dropout}.}
% analogous to spatial dropout \cite{tompson2015efficient} but operating along the time axis. 
By training on disordered sequences, the generator learns to recover plausible trajectories, effectively regularizing temporal entropy. FluxFlow is grounded in two principles:
\begin{itemize}[leftmargin=*]
    \item[\ding{238}] \textbf{Disentanglement via Perturbation}: Shuffling disrupts spurious correlations (\textit{e.g.}, ``frame order $=$ motion causality"), forcing the model to infer latent transition probabilities between states. This aligns with evidence from video understanding \cite{yang2020temporal, huang2025sefar, singh2021semi, xing2023svformer}, where temporal augmentations improve motion representation learning.
    \item[\ding{238}] \textbf{Implicit Curriculum Learning}: Progressive shuffling mimics human skill acquisition: early stages focus on coarse motion structure, while later stages refine fine-grained dynamics.
\end{itemize}

FluxFlow bridges the gap between discriminative and generative temporal augmentation, offering a plug-in solution for temporal plausible video generation. To summarize, our contributions are as follows:
\begin{itemize}[leftmargin=*]
    \item We introduce \textbf{FluxFlow}, the first dedicated temporal augmentation strategy for video generation, requiring no architectural changes.
    \item We formalize temporal shuffling as a variational regularization problem, showing it bounds the generator’s entropy over motion paths.
    \item Extensive experiments demonstrate ...
\end{itemize}

